PointGMM: a Neural GMM Network for Point Clouds

Point clouds are a popular representation for 3D shapes. However, they encode a particular sampling without accounting for shape priors or non-local information. We advocate for the use of a hierarchical Gaussian mixture model (hGMM), which is a compact, adaptive and lightweight representation that probabilistically defines the underlying 3D surface. We present PointGMM, a neural network that learns to generate hGMMs which are characteristic of the shape class, and also coincide with the input point cloud. PointGMM is trained over a collection of shapes to learn a class-specific prior. The hierarchical representation has two main advantages: (i) coarse-to-fine learning, which avoids converging to poor local-minima; and (ii) (an unsupervised) consistent partitioning of the input shape. We show that as a generative model, PointGMM learns a meaningful latent space which enables generating consistent interpolations between existing shapes, as well as synthesizing novel shapes. We also present a novel framework for rigid registration using PointGMM, that learns to disentangle orientation from structure of an input shape.

==> dispracted0301_hgmm.tex <==
\subsection{Hierarchical GMM}
\label{sec:hgmm}
\rh{
% the main idea
The \hgm{} is a distribution defined by a set of Gaussians in a tree structure. 
Each node in the tree has a GMM associated with it, and a hierarchical lineage. \ahc{In order to calculate the log-likelihood of a given point cloud in the \hgm{} distribution} We recursively partition each point in the point cloud $x \in X$ by the probabilities of the nodes in the tree, and generate GMM parameters for each distinct subset of points. 
}
A parent node $n_j$ defines a GMM by its children $Ch(n_j)$.
% $Si(\node{})$--- nodes that share the same parent as $\node{}$. 
Each child node $n_i$ corresponds to a Gaussian in the mixture with the parameters $\Theta_{\ind{}} = \left \{\pi_\ind{}, \mu_\ind{}, \Sigma_\ind{}\right\}$. Thus, the probability density function is given by $p\left(x \vert \Theta_i\right) = \pi_i \cdot \normal{x}{i}$ 
with mixture weights $\sum_{n_{i} \in Ch(n_j)}\pi_{i} = 1.$


% The Gaussian parameters are mixed between sibling nodes, \emph{i.e.,} nodes which share the same parent. 
% The GMM parameters for the $j^{th}$ group of siblings is given by $\Theta_{j} = \left\{\pi_\ind{}, \mu_\ind{}, \Sigma_\ind{}\right\}_{\ind{} \in \mathcal{S}_j}$, where $\mathcal{S}_j$ is the set of siblings.
% The probability that a point $x \in \pc$ came from the distribution $\Theta_j$ is 
% \begin{equation}
%     p\left(x \vert \Theta_j\right) = \sum_{i \in \mathcal{S}_j} \pi_\ind{} \cdot \normal{x}{\ind{}}.
% \end{equation}
% }
% A child node 
% Each child node $\node{}$ (at depth $i$) \textit{Sibling} nodes



\textbf{Log-Likelihood.} 
Given a point cloud $\pc$, we calculate its log-likelihood For each depth in the hierarchy. We follow the hard-partition log-likelihood \cite{eckart2016accelerated}, where we recursively partition \ah{the point cloud $\pc$} across the nodes of the tree, and then consider each node as a separate GMM distribution. Therefore, each point in the point-cloud is partitioned into a distinct parent node at each depth, recursively.
A point will be partitioned to a node $\n_j$ if it is the most likely that it came from its from its correspond Gaussian among its siblings $Si(n_j)$ (children with the same parent):
\begin{equation}
\pr\left(\pc{}, n_j\right) = \{x\in \pc \vert j = \argmax{i \in Si(n_j)} p\left(x \vert \Theta_i\right) \}.
\end{equation}
% For a group of siblings $\mathcal{S}_j$ (children with the same parent) {we calculate the density function $p\left(x \vert \Theta_j\right)$ for each point $x \in \pc$} and select the child with the largest probability:



%
%
% This is done by selecting the child $n_\ind{}$ with the largest probability density $p\left(x \vert \Theta\left(n_\ind{}\right)\right)$ to represent $x$ among its siblings, which given by
% \begin{equation}
% \pr\left(\pc{}, \node{}\right) = \{x\in \pc \vert \node{} = \argmax{n_{i,l}\in Si(\node{})}p\left(x \vert \Theta(n_{i,l})\right) \}.
% \end{equation}

We use each point partition 
% \rgc{I think it is wrong. It should be the log-likelihood at depth $d$ associated with the subtree of node $\node{}$. This sentence appears after the formula but I believe should be moved here.} 
associated with node $n_j$ at depth $\depth{}$ to calculate the log-likelihood for the \hgm{} $ \ell\left(\pc, \depth{},n_{j} \vert \Theta \right)$. The likelihood can be calculated recursively by:
\begin{multline}
 \ell\left(\pc, \depth{}, n_j \vert \Theta \right) = \\
 \begin{cases} \sum\limits_{x \in \pc}\log{\sum\limits_{i \in Ch(n_{j})}p\left(x \vert \Theta\left(n_{i}\right)\right)} &\mbox{if } j = \depth{}  \\ 
 \sum_{i \in Ch(n_i)} \ell\left(\pr \left(\pc, n_i\right), \depth{}, n_{j} \vert \Theta \right) & \mbox{else}.
 \end{cases}
\end{multline}

This definition, provides us with the log-likelihood \ah{(calculated using by sibling GMMs groups of depth $d+1$)} associated with the sub-tree of node $\node{}$. 
Thus, the log-likelihood of the whole tree (with the GMMs of depth $d$), is simply given by $$\ell\left(\pc, \depth{} \vert \Theta \right) \triangleq \ell\left(\pc, \depth{}, \nr \vert \Theta \right),$$
where $\nr$ is the root node \ah{and $1 \leq d < D$ where $D$ is the tree depth.}

Since the \hgm{} log-likelihood is differentiable, it can be used as the loss function for training \ourmethod{} to generate a \hgm{} from a given point cloud.

\rhc{remember to change the indices to be consistent if you agree with my new notation.}

